Network Thermodynamical Modelling of Bioelectrical Systems: A Bond Graph Approach

Interactions between biomolecules, electrons and protons are essential to many fundamental processes sustaining life. It is therefore of interest to build mathematical models of these bioelectrical processes not only to enhance understanding but also to enable computer models to complement in vitro and in vivo experiments.Such models can never be entirely accurate; it is nevertheless important that the models are compatible with physical principles. Network Thermodynamics, as implemented with bond graphs, provide one approach to creating physically compatible mathematical models of bioelectrical systems. This is illustrated using simple models of ion channels, redox reactions, proton pumps and electrogenic membrane transporters thus demonstrating that the approach can be used to build mathematical and computer models of a wide range of bioelectrical systems.

==> BG-defs.tex <==
%% Referencing and indexing
%%\newcommand{\Index}[1]{\emph{#1}\index{\MakeLowercase{#1}}}
\newcommand{\Index}[1]{\emph{#1}\index{#1}}
\newcommand{\IndeX}[1]{\emph{#1}\index{#1}}
\newcommand{\Ref}[1]{\ref{#1}, p.\pageref{#1}}
\newcommand{\cref}[1]{Chapter~\Ref{#1}}
\newcommand{\aref}[1]{Appendix~\Ref{#1}}
\newcommand{\sref}[1]{\S~\Ref{#1}}
\newcommand{\fref}[1]{Figure~\Ref{#1}}
\newcommand{\eref}[1]{Equation~\eqref{#1}}
\newcommand{\nitem}[3]{\item[#1] #2 \sref{#3}\index{#1}}
\newcommand{\eoe}{$\bm{\Diamond}$} % End of example mark.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "book"
%%% End:

